Sparse Recovery Beyond Compressed Sensing: Separable Nonlinear Inverse Problems

Extracting information from nonlinear measurements is a fundamental challenge in data analysis. In this work, we consider separable inverse problems, where the data are modeled as a linear combination of functions that depend nonlinearly on certain parameters of interest. These parameters may represent neuronal activity in a human brain, frequencies of electromagnetic waves, fluorescent probes in a cell, or magnetic relaxation times of biological tissues. Separable nonlinear inverse problems can be reformulated as underdetermined sparse-recovery problems, and solved using convex programming. This approach has had empirical success in a variety of domains, from geophysics to medical imaging, but lacks a theoretical justification. In particular, compressed-sensing theory does not apply, because the measurement operators are deterministic and violate incoherence conditions such as the restricted-isometry property. Our main contribution is a theory for sparse recovery adapted to deterministic settings. We show that convex programming succeeds in recovering the parameters of interest, as long as their values are sufficiently distinct with respect to the correlation structure of the measurement operator. The theoretical results are illustrated through numerical experiments for two applications: heat-source localization and estimation of brain activity from electroencephalography data.

==> algorithms.tex <==
\section{Algorithms}

\subsection{Robustness}




==> eeg.tex <==
\subsection{Localization of Brain Activity using Electronencephalography}
\label{sec:eeg}

It is important to measure brain activity because ???. Electroencephalography (EEG) measurements of the electric potential field on the surface of the head~\cite{niedermeyer2005eeg} can be used to detect regions of focalized activity in the brain. Under certain assumptions (what assumptions???), the data follow an SNL model where the parameters are the locations of these regions. The function $\phi_t\brac{\theta}$ represents the potential at a specific location $t$ of the head produced by a dipole (why a dipole? maybe just cite something??) at position $\theta$ in the brain. This function can be computed by solving the Poisson differential equation (write it down) taking into account the geometry and electric properties (what properties??? conductivities of different tissues) of the head~\cite{nunez2006electric}. Explain a bit about geometry. 

\begin{figure}[H]
\centering
\includegraphics[width=8cm]{./figs/eeg_exp/results_50_best.eps}
\includegraphics[width=8cm]{./figs/eeg_exp/results_50_worst.eps}
\caption{Results of 50 points, Left, best case, right worst case}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=8cm]{./figs/eeg_exp/results_60_best.eps}
\includegraphics[width=8cm]{./figs/eeg_exp/results_60_worst.eps}
\caption{Results of 60 points, Left, best case, right worst case}
\end{figure}

We conduct a numerical experiment on EEG data. In our experiment, three simulated dipoles are inserted such that their mutual Euclidean distances are similar. To achieve this, a series of distance values are first linearly obtained in the range from the minimum distance to the maximum distance between any two locations. Then for a specific distance value, we uniformly select a dipole location and find other two dipoles having the most similar mutual distances and their values are close to that specific distance value. For amplitudes of the signal, we tried all sign combinations with magnitudes equal to 1, we declare fail as long as one of the cases is failed to be solved. We repeatedly simulate instances for 60 distance values. 

%EEG source-localization techniques aim to detect areas of focalized brain activity from measurements of the electric potential field on the surface of the head~\cite{niedermeyer2005eeg}. Under the common assumption that the number of active areas is small, the data can be expressed in terms of a sparse linear model~\cite{silva2004evaluation,xu2007lp}. Each atom in the dictionary contains the field values generated by an electric source located at a specific position, which can be obtained by computing the Green's function of the Poisson differential equation governing the field~\cite{nunez2006electric}. Nonzero coefficients in the model reveal active locations in the brain. 

% http://www.scholarpedia.org/article/Source_localization
% http://www.scholarpedia.org/article/Electroencephalogram
% http://www.nmr.mgh.harvard.edu/meg/pdfs/1993-Hamalainen-RMP.pdf


==> heat.tex <==
\subsection{Heat-Source Localization}
\label{sec:heat}
Consider the heat equation on $[0,1]$ with varying conductivity and
Neumann boundary conditions \cite{li2014heat}:
\begin{align}
  \frac{\partial}{\partial t}u(x,t) &= \frac{\partial}{\partial
    x}\left(a(x)\frac{\partial}{\partial x}u(x,t)\right),\\
  \frac{\partial}{\partial x}u(0,t) &= \frac{\partial}{\partial
    x}u(1,t) = 0.
\end{align}
The function $a$ controls the conductivity of the underlying medium.
Regions where $a$ is large allow for heat to diffuse quickly.
At a fixed time $T=10^{-4}$ we measure the heat $u(j/100,T)$ for
$j=0,\ldots,100$.  Using these samples we must recover the initial
heat distribution at time $t=0$: a collection of point sources of
heat of the form
\begin{equation}
  x = \sum_{\theta_i\in\Theta} c_i\delta_{\theta_i},
\end{equation}
where $\Theta$ is a finite subset of $[0,1]$ and
$c_i\in\RR$ for $i=1,\ldots,|\Theta|$.

To put this problem into the form of \eqref{pr:min_l1} we discretize
the interval $[0,1]$ into the grid $\{j/N\}_j$ for $j=0,\ldots,N$
where $N>0$ is fixed.
We construct each column $\vphi(j/N)$ of $\Phi$ by numerically
solving the heat equation using a finite difference method with initial
condition $x=\delta_{j/N}$.  In \Cref{fig:} we
show an example of the conductivity, initial conditions, samples, and the measure
recovered using \eqref{pr:min_l1}.  Using $\ell_1$-minimization for
heat-source localization was studied in \cite{li2014heat}, where they
present numerical examples, and prove recovery results for a single
source.


==> mrf.tex <==
\subsection{Estimation of Magnetic-Resonance Relaxation Times}
\label{sec:mrf}
Magnetic resonance imaging (MRI) is a medical-imaging modality based on the nuclear magnetic-resonance phenomenon, in which the spin of certain atomic nuclei absorb and emit electromagnetic radiation. To perform MRI, subjects are placed in a strong magnetic field that generates a macroscopic net magnetization of the nuclear spins in their bodies. Radio-frequency (RF) pulses are used to manipulate this magnetization, causing it to precess. % As a result, an electromagnetic signal is emitted, which is measured and processed. 
The dynamics of the magnetization are governed by the Bloch equation~\cite{bloch1946nuclear}:
\begingroup
 \renewcommand{\arraystretch}{1.4}
 \begin{equation}
\frac{\partial}{\partial t} \begin{pmatrix}M_x \\ M_y \\ M_z \end{pmatrix} = \begin{pmatrix} \omega_x \\ \omega_y \\ \omega_z \end{pmatrix} \times \begin{pmatrix}M_x \\ M_y \\ M_z \end{pmatrix} - \begin{pmatrix}\frac{M_x}{T_2} \\ \frac{M_y}{T_2} \\ \frac{M_z - 1}{T_1} \end{pmatrix},
\label{eq:Bloch}
\end{equation}
\endgroup
where $\partial / \partial t$ is a partial derivative with respect to time. $M_x$,  $M_y$ and $M_z$ are functions of time which denote the magnetization along the three spatial dimensions. The Larmor frequency $\omega_z$ is the frequency at which the spins precess. Magnetic fields, called \emph{gradient fields} because they vary linearly along different spatial dimensions, are used to modify $\omega_z$ and select the specific region to be imaged, as well as to encode the magnetization in the Fourier domain. The frequencies $\omega_x$ and $\omega_y$ are varied over time using RF pulses in order to create a specific spin evolution that makes spin-relaxation effects accessible. This evolution is determined by the relaxation times $T_1$ and $T_2$. We refer to~\cite{nishimura1996principles} for more details on MRI models and methods.

In traditional MRI, acquisition is designed so that the resulting signal at each voxel of an image is predominantly weighted by the $T_1$ or $T_2$ relaxation times of the tissues present in the voxel. MR images obtained in this way are qualitative in nature: they consist of gray values that capture relative signal intensity changes between tissues, caused by their different $T_1$ and $T_2$ values, which are then interpreted by radiologists to detect pathologies. The specific numerical value at each voxel is typically subject to variations between different MRI systems and data-acquisition settings. As a result, it is very challenging to use current clinical MRI systems for longitudinal studies and computer-aided diagnosis. The goal of quantitative MRI is to measure physical parameters such as $T_1$ and $T_2$ quantitatively, in a way that is \emph{reproducible} across different MRI systems~\cite{giedd1996quantitative,suddath1989temporal,tofts2005quantitative}. 
% Quantitative MRI techniques can be used to extract  biomarkers for medical diagnostics~\cite{reich2007multiparametric,matzat2013quantitative,neema2007t1} and synthesize images with standardized contrasts~\cite{noth2015improved,Deshmane2016}. 

Magnetic resonance fingerprinting (MRF) \cite{ma2013magnetic} is a recently-proposed technique to measure the relaxation times $T_1$ and $T_2$ quantitatively. Instead of driving the magnetization into a steady state with a fixed weighting of $T_1$ and $T_2$ effects, MRF acquisition is designed to produce highly irregular magnetization signals, from which $T_1$ and $T_2$ can be estimated robustly. If a voxel contains only one tissue, the time evolution of the magnetization measured at the voxel is a solution $\phi_t\brac{T_1, T_2}$ to the Bloch equation~\eqref{eq:Bloch} parametrized by the $T_1$ and $T_2$ values of the tissue. If there are several tissues in the voxel, the magnetization can be modeled as an additive superposition of such functions, weighted by a coefficient that represents the contribution of each tissue~\cite{McGivney2017,mcmrf}, as long as the chemical exchange between the tissue compartments~\cite{Allerhand1964} can be neglected. This is an SNL model where $k$ is the number of tissues and the parameters $\theta_1$, \ldots, $\theta_k$ are two-dimensional: they represent the $T_1$ and $T_2$ relaxation times of each tissue. 


==> proofstuff.tex <==
\section{Proof stuff}
\subsection{Dual Certificates when $p=1$}
When $p=1$ the dual combination $Q$ takes the form
$$Q(\theta) = \sum_{i=1}^{|\Theta|}\alpha_i\rho(\theta_i,\theta) +
\beta_i\rho^{(1,0)}(\theta_i,\theta),$$
where $\rho^{(q,r)}$ denotes $q$ derivatives with respect to the first
argument, and $r$ derivatives with respect to the second.
In order to satisfy conditions \eqref{eq:certinterp} and
\eqref{eq:certbound} of \Cref{thm:dualcert},
$Q$ must interpolate the points $(\theta_j,\sigma_j)$ for
$\theta_j\in\Theta$ and have local
extrema at each such point.  These give rise to the following
``interpolation equations'':
\begin{align}
  \sigma_j &= \sum_{i=1}^{|\Theta|}
  \alpha_i\rho(\theta_i,\theta_j)+\beta_i\rho^{(1,0)}(\theta_i,\theta_j)\label{eq:interp1}\\
  0 &=\sum_{i=1}^{|\Theta|}
  \alpha_i\rho^{(0,1)}(\theta_i,\theta_j)+\beta_i\rho^{(1,1)}(\theta_i,\theta_j).\label{eq:interp2}
\end{align}

To gain some intuition into the $\alpha,\beta$-values, consider the scenario where $\rho(\theta,\eta)$ and
$\rho^{(1,0)}(\theta,\eta)$ decay as $|\theta-\eta|$ grows and
where $|\theta_i-\theta_j|$ is sufficiently large for all
$\theta_i,\theta_j\in\Theta$ where $i\neq j$.
Note that $\rho(\theta_j,\theta_j)=1$ and
$$\rho^{(1,0)}(\theta_j,\theta_j) = \rho^{(0,1)}(\theta_j,\theta_j)
=\Phi^{(1)}(\theta_j)^T\Phi(\theta_j)=0,$$
which follows from our convention that $\normTwo{\Phi(\theta)}^2=1$.  Equation
\eqref{eq:interp1} then implies
that $\alpha_j\approx\sigma_j$.  Using equation \eqref{eq:interp2} we
see that the $\beta$-values are used to correct any deviations of the
derivatives from zero at the $\theta_j$ values.  The magnitude of
$\beta_i$ is inversely proportional to the quantity
$\rho^{(1,1)}(\theta_i,\theta_i)=\normTwo{\Phi^{(1)}(\theta_i)}^2$.
We expect $\normTwo{\Phi^{(1)}(\theta_i)}$ to be bounded away from zero
when the recovery problem is well-posed, as otherwise small changes in
parameter space are not reflected in the features.

Define $\epsilon_i^{(q,r)}(s)$ by
$$\epsilon_i^{(q,r)}(\theta) := \sum_{j\neq
  i}\left|\frac{\rho^{(q,r)}(\theta_j,\theta)}{\rho^{(q,q)}(\theta_j,\theta_j)}\right|
= \sum_{j\neq
  i}\frac{|\Phi^{(q)}(\theta_j)^T\Phi^{(r)}(\theta)|}{\|\Phi^{(q)}(\theta_j)\|_2^2},$$
where $q\in\{0,1\}$. Here we think of $\theta$ as a point close to
$\theta_i$ so that $\epsilon_i^{(q,r)}(s)$ captures the correlation
effects from the other, distant elements of $\Theta$.  We expect
$\epsilon_i^{(q,r)}(s)$ to be small when $\rho$ has sufficient decay
and $\Theta$ is well-separated.  Below we show that bounds on
$\epsilon_i^{(q,r)}$ imply exact recovery.

By normalizing the $\beta_i$ coefficients, we can rewrite our dual certificate as
\begin{equation}
  Q(\theta) = \sum_{i=1}^{|\Theta|}
  \alpha_i\rho(\theta_i,\theta)+\beta_i\frac{\rho^{(1,0)}(\theta_i,\theta)}{\rho^{(1,1)}(\theta_i,\theta_i)}. \label{eq:normdualcert}
\end{equation}
Then the interpolation equations \eqref{eq:interp1},
\eqref{eq:interp1} applied to \eqref{eq:normdualcert} give the system
\begin{equation}
  \MAT{\II+P^{(0,0)}&P^{(1,0)}\\P^{(0,1)}&\II+P^{(1,1)}}\MAT{\alpha\\\beta}=\MAT{\sigma\\0},\label{eq:interpmat}
\end{equation}
where $\II\in\RR^{|\Theta|\times|\Theta|}$ is the identity matrix, and
$P^{(q,r)}\in\RR^{|\Theta|\times|\Theta|}$ satisfies
$$P^{(q,r)}_{ij} = \rho^{(q,r)}(\theta_j,\theta_i)/\rho^{(q,q)}(\theta_j,\theta_j)$$
for $i\neq j$ and $P^{(q,r)}_{ii}=0$. Our definition above gives
$$\|P^{(q,r)}\|_\infty =
\max_{i\in\{1,\ldots,|\Theta|\}}\epsilon_i^{(q,r)}(\theta_i)=:\epsilon^{(q,r)}.$$
Analyzing Schur complements allows us to bound $\alpha$ and $\beta$ in
terms of $\epsilon^{(q,r)}$.
\begin{lemma}
  \label{thm:schurbound}
  Suppose $\epsilon^{(1,1)}<1$ and
  \begin{equation}
    \epsilon^{(0,0)}+\frac{\epsilon^{(1,0)}\epsilon^{(0,1)}}{1-\epsilon^{(1,1)}}<1.
  \end{equation}
  Then equation \eqref{eq:normdualcert} is invertible and
  \begin{align}
    \|\alpha\|_\infty
    & \leq
    \frac{1}{1-(\epsilon^{(0,0)}+\epsilon^{(1,0)}\epsilon^{(0,1)}/(1-\epsilon^{(1,1)}))}
    =
    \frac{1-\epsilon^{(1,1)}}{(1-\epsilon^{(0,0)})(1-\epsilon^{(1,1)})-\epsilon^{(1,0)}\epsilon^{(0,1)}}\\
    \|\beta\|_\infty
    & \leq
    \frac{\epsilon^{(0,1)}/(1-\epsilon^{(1,1)})}{1-(\epsilon^{(0,0)}+\epsilon^{(1,0)}\epsilon^{(0,1)}
      /(1-\epsilon^{(1,1)}))}  =
    \frac{\epsilon^{(0,1)}}{(1-\epsilon^{(0,0)})(1-\epsilon^{(1,1)})-\epsilon^{(1,0)}\epsilon^{(0,1)}}\\
    \aLB
    & \geq 2 -
    \frac{1}{1-(\epsilon^{(0,0)}+\epsilon^{(1,0)}\epsilon^{(0,1)}/(1-\epsilon^{(1,1)}))}=
    2 - \frac{1-\epsilon^{(1,1)}}{(1-\epsilon^{(0,0)})(1-\epsilon^{(1,1)})-\epsilon^{(1,0)}\epsilon^{(0,1)}}.
  \end{align}
  Above $\aLB$ denotes a quantity such that $|\alpha_i|\geq \aLB$ for
  all $i$.
\end{lemma}
Applying the triangle inequality immediately gives the following
bounds on $Q$.
\begin{lemma}
  \label{thm:dualcertbound}
  Fix $\theta_i\in\Theta$ and let $Q$ be defined as in \eqref{eq:normdualcert}.  For all $\theta\in\RR$
  \begin{equation}
    |Q(\theta)|
    \leq
    \|\alpha\|_\infty|\rho(\theta_i,\theta)|+\|\beta\|_\infty\left|\frac{\rho^{(1,0)}(\theta_i,\theta)}{\rho^{(1,1)}(\theta_i,\theta_i)}\right|
    + \|\alpha\|_\infty
    \epsilon_i^{(0,0)}(\theta)+\|\beta\|_\infty\epsilon_i^{(1,0)}(\theta).
  \end{equation}
  If $\rho^{(0,1)}(\theta)\leq0$ then
  \begin{equation}
    Q'(\theta)
    \leq
    \aLB\rho^{(0,1)}(\theta_i,\theta)+\|\beta\|_\infty\left|\frac{\rho^{(1,1)}(\theta_i,\theta)}{\rho^{(1,1)}(\theta_i,\theta_i)}\right|
    + \|\alpha\|_\infty
    \epsilon_i^{(0,1)}(\theta)+\|\beta\|_\infty\epsilon_i^{(1,1)}(\theta).
  \end{equation}
  If $\rho^{(0,2)}(\theta_i,\theta)\leq0$ then
  \begin{equation}
    Q''(\theta)\leq
    \aLB\rho^{(0,2)}(\theta_i,\theta)+\|\beta\|_\infty\left|\frac{\rho^{(1,2)}(\theta_i,\theta)}{\rho^{(1,1)}(\theta_i,\theta_i)}\right|
    + \|\alpha\|_\infty
    \epsilon_i^{(0,2)}(\theta)+\|\beta\|_\infty\epsilon_i^{(1,2)}(\theta).
  \end{equation}
\end{lemma}
These bounds, when combined with the following lemma, give us an
effective method for proving exact recovery.
\begin{lemma}
  \label{thm:taylorbound}
  Let $f:\RR\to\RR$ with $f\in\cC^2$ and suppose there are
  $0<u_1\leq u_2\leq h$ with
  \begin{enumerate}
  \item $f(0)=1$
  \item $f''(t) < 0$ for $t\in [0,u_1]$,
  \item $f'(t) < 0$ for $t\in[u_1,u_2]$,
  \item and $|f(t)|<1$ for $t\in[u_2,h]$.
  \end{enumerate}
  Then $|f(t)|<1$ for $t\in (0,h]$.
\end{lemma}
There are several ways to trade off the accuracy of the above exact
recovery method in order to obtain a cleaner condition on recovery.
These include assuming $\rho$ has a particular functional form,
that $\rho$ and its derivatives are bounded by a
decaying envelope, or that $\rho$ and its derivatives have
piecewise-constant bounds.  Such conditions have been explored in
other papers in a variety of other contexts.
Here we will use the $p=2$ version of the above results to
directly to analyze exact recovery in the setting of EEG, MRF, and DoA.

\subsubsection{Dual Certificates when $p=2$}
In this section, we briefly show how the one dimensional results
extend to the two dimensional case.  Due to the extra variables, we
now require a more cumbersome notation for partial derivatives.
We write $\rho^{(q,r,s,t)}(\eta,\zeta)$ where $q,r$ are the number of
derivatives with respect to the first and second coordinates of
$\eta$, and $s,t$ are with respect to the first and second coordinates
of $\zeta$.  As above, we define
\begin{equation}
  \epsilon_i^{(q,r,s,t)}(\theta) := \sum_{j\neq
  i}\left|\frac{\rho^{(q,r,s,t)}(\theta_j,\theta)}{\rho^{(q,r,q,r)}(\theta_j,\theta_j)}\right|
= \sum_{j\neq
  i}\frac{|\Phi^{(q,r)}(\theta_j)^T\Phi^{(s,t)}(\theta)|}{\|\Phi^{(q,r)}(\theta_j)\|_2^2},
\end{equation}
where $q+r\leq 1$ and $s+t\leq 2$.  As above, we expect the
denominator to be bounded away from zero when the recovery problem is
well-posed.  The new constraint we observe when $p=2$ is that the
following quantity is small
\begin{equation}
  |\Phi^{(1,0)}(\theta_j)^T\Phi^{(0,1)}(\theta_j)|.
\end{equation}
If this doesn't hold, then changes to each coordinate of $\theta_j$
perturb the feature vector $\Phi(\theta_j)$ along a similar
direction.  This creates ambiguity that effects the well-posedness of
the recovery problem.

Our dual combination $Q$ now takes the form
\begin{equation}
  \label{eq:normdualcert_p2}
  Q(\theta) = \sum_{i=1}^{|\Theta|}\alpha_i\rho(\theta_i,\theta) +
  \beta_i\frac{\rho^{(1,0,0,0)}(\theta_i,\theta)}{\rho^{(1,0,1,0)}(\theta_i,\theta_i)}+\kappa_i\frac{\rho^{(0,1,0,0)}(\theta_i,\theta)}{\rho^{(0,1,0,1)}(\theta_i,\theta_i)},
\end{equation}
and the interpolation equations take the form
\begin{align}
  \sigma_j &= \sum_{i=1}^{|\Theta|}
  \alpha_i\rho(\theta_i,\theta_j)
  +\beta_i\frac{\rho^{(1,0,0,0)}(\theta_i,\theta)}{\rho^{(1,0,1,0)}(\theta_i,\theta_i)}
  +\kappa_i\frac{\rho^{(0,1,0,0)}(\theta_i,\theta)}{\rho^{(0,1,0,1)}(\theta_i,\theta_i)}
  \label{eq:interp1_p2}\\
  0 &= \sum_{i=1}^{|\Theta|}
  \alpha_i\rho^{(0,0,1,0)}(\theta_i,\theta_j)
  +\beta_i\frac{\rho^{(1,0,1,0)}(\theta_i,\theta)}{\rho^{(1,0,1,0)}(\theta_i,\theta_i)}
  +\kappa_i\frac{\rho^{(0,1,1,0)}(\theta_i,\theta)}{\rho^{(0,1,0,1)}(\theta_i,\theta_i)}
  \label{eq:interp2_p2}\\
  0 &= \sum_{i=1}^{|\Theta|}
  \alpha_i\rho^{(0,0,0,1)}(\theta_i,\theta_j)
  +\beta_i\frac{\rho^{(1,0,0,1)}(\theta_i,\theta)}{\rho^{(1,0,1,0)}(\theta_i,\theta_i)}
  +\kappa_i\frac{\rho^{(0,1,0,1)}(\theta_i,\theta)}{\rho^{(0,1,0,1)}(\theta_i,\theta_i)}
  \label{eq:interp3_p2},
\end{align}
for all $\theta_j\in\Theta$.  In matrix form, this becomes
\begin{equation}
  \MAT{
    \II+P & P^{(1,0,0,0)} & P^{(0,1,0,0)}\\
    P^{(0,0,1,0)} & \II+P^{(1,0,1,0)} & \DD^{(0,1,1,0)}+P^{(0,1,1,0)}\\
    P^{(0,0,0,1)} & \DD^{(1,0,0,1)}+P^{(1,0,0,1)} & \II+P^{(0,1,0,1)}
  }
  \MAT{\alpha\\\beta\\\kappa}
  =\MAT{\sigma\\0\\0}.
\label{eq:interpmat_p2}
\end{equation}
Here $P\in\RR^{|\Theta|\times|\Theta|}$ is defined as above such that
\begin{equation}
  P^{(q,r,s,t)}_{ij}=
  \frac{\rho^{(q,r,s,t)}(\theta_i,\theta_j)}{\rho^{(q,r,q,r)}(\theta_i,\theta_i)}
\end{equation}
for $i\neq j$ and $P^{(q,r,s,t)}_{ii}=0$.
Likewise $\DD^{(q,r,s,t)}\in\RR^{|\Theta|\times|\Theta|}$ is a diagonal matrix with
\begin{equation}
  \DD^{(q,r,s,t)}_{ii}=
  \frac{\rho^{(q,r,s,t)}(\theta_i,\theta_i)}{\rho^{(q,r,q,r)}(\theta_i,\theta_i)}.
\end{equation}
As before we obtain
$$\|P^{(q,r,s,t)}\|_\infty =
\max_{i\in\{1,\ldots,|\Theta|\}}\epsilon_i^{(q,r,s,t)}(\theta_i)=:\epsilon^{(q,r,s,t)}.$$
This leads to the following bounds.
\bdb{Haven't computed the schur bound yet}
\begin{lemma}
  \label{thm:schurbound_p2}
  Suppose $\epsilon^{(1,1)}<1$ and
  \begin{equation}
    \epsilon^{(0,0)}+\frac{\epsilon^{(1,0)}\epsilon^{(0,1)}}{1-\epsilon^{(1,1)}}<1.
  \end{equation}
  Then equation \eqref{eq:interpmat_p2} is invertible and
  \begin{align}
    \|\alpha\|_\infty
    & \leq\\
    \|\beta\|_\infty
    & \leq\\
    \|\kappa\|_\infty
    & \leq\\
    \aLB
    & \geq.
  \end{align}
  Above $\aLB$ denotes a quantity such that $|\alpha_i|\geq \aLB$ for
  all $i$.
\end{lemma}
To complete our treatment of $p=2$, fix $\theta$ and let
$\theta_i\in\Theta$ be the closest element of $\Theta$ to $\theta$.
To apply \Cref{thm:taylorbound} in a 2-dimensional setting, we
consider the line from $\theta_i$ to $\theta$ and bound $Q$
accordingly.  More precisely, we define $f:\RR\to\RR$ by
\begin{align}
  f(t) &= Q(\theta_i + t(\theta-\theta_i))\\
  f'(t) &= \nabla Q(\theta_i + t(\theta-\theta_i))^T(\theta-\theta_i)\\
  f''(t) &= (\theta-\theta_i)^T\nabla^2Q(\theta_i + t(\theta-\theta_i))(\theta-\theta_i).
\end{align}
If we can prove $|Q|<1$ on all radial lines emitted from
each $\theta_i\in\Theta$ the result follows.  This leads to the
following analog of \Cref{thm:dualcertbound}.  Below we use the
notation
\begin{equation}
  \epsilon_i^{(q,r,\nabla)}(\theta)=
  \MAT{\epsilon_i^{(q,r,1,0)}(\theta)\\\epsilon_i^{(q,r,0,1)}(\theta)}
  ,\quad
  \epsilon_i^{(q,r,\nabla^2)}(\theta)=
  \MAT{
    \epsilon_i^{(q,r,2,0)}(\theta) & \epsilon_i^{(q,r,1,1)}(\theta)\\
    \epsilon_i^{(q,r,1,1)}(\theta) & \epsilon_i^{(q,r,0,2)}(\theta)
  },
\end{equation}
and similarly for $\rho$.
\begin{lemma}
  \label{thm:dualcertbound_p2}
  Fix $\theta_i\in\Theta$ and let $Q$ be defined as in
  \eqref{eq:normdualcert_p2}.  Fix $\theta\in\RR^2$ and define $d$ by
  $$d:= \frac{\theta-\theta_i}{\|\theta-\theta_i\|_2}.$$
  Then we have
  \begin{align}
    |Q(\theta)|
    &\leq
    \|\alpha\|_\infty|\rho(\theta_i,\theta)|+\|\beta\|_\infty\left|\frac{\rho^{(1,0,0,0)}(\theta_i,\theta)}{\rho^{(1,0,1,0)}(\theta_i,\theta_i)}\right|
    +\|\kappa\|_\infty\left|\frac{\rho^{(0,1,0,0)}(\theta_i,\theta)}{\rho^{(0,1,0,1)}(\theta_i,\theta_i)}\right|\nonumber\\
    &+ \|\alpha\|_\infty
    \epsilon_i^{(0,0,0,0)}(\theta)+\|\beta\|_\infty\epsilon_i^{(1,0,0,0)}(\theta)+\|\kappa\|_\infty\epsilon_i^{(0,1,0,0)}(\theta).
  \end{align}
  If $\rho^{(0,0,\nabla)}_i(\theta)^Td\leq 0$ then
  \begin{align}
    \nabla Q(\theta)^Td
    &\leq
    \aLB\rho^{(0,0,\nabla)}(\theta_i,\theta)^Td
    +\|\beta\|_\infty\left\|\frac{\rho^{(1,0,\nabla)}(\theta_i,\theta)}{\rho^{(1,0,1,0)}(\theta_i,\theta_i)}\right\|_2
    +\|\kappa\|_\infty\left\|\frac{\rho^{(0,1,\nabla)}(\theta_i,\theta)}{\rho^{(0,1,0,1)}(\theta_i,\theta_i)}\right\|_2\nonumber\\
    &+ \|\alpha\|_\infty
    \|\epsilon_i^{(0,0,\nabla)}(\theta)\|_2+\|\beta\|_\infty\|\epsilon_i^{(1,0,\nabla)}(\theta)\|_2+\|\kappa\|_\infty\|\epsilon_i^{(0,1,\nabla)}(\theta)\|_2.
  \end{align}
  If $d^T\rho^{(0,0,\nabla^2)}(\theta_i,\theta)d\leq0$ then
  \begin{align}
    d^T\nabla^2Q(\theta)d
    &\leq
    \aLB d^T\rho^{(0,0,\nabla^2)}(\theta_i,\theta)d
    +\|\beta\|_\infty\left\|\frac{\rho^{(1,0,\nabla^2)}(\theta_i,\theta)}{\rho^{(1,0,1,0)}(\theta_i,\theta_i)}\right\|_2
    +\|\kappa\|_\infty\left\|\frac{\rho^{(0,1,\nabla^2)}(\theta_i,\theta)}{\rho^{(0,1,0,1)}(\theta_i,\theta_i)}\right\|_2\nonumber\\
    &+ \|\alpha\|_\infty
    \|\epsilon_i^{(0,0,\nabla^2)}(\theta)\|_2+\|\beta\|_\infty\|\epsilon_i^{(1,0,\nabla^2)}(\theta)\|_2+\|\kappa\|_\infty\|\epsilon_i^{(0,1,\nabla^2)}(\theta)\|_2,
  \end{align}
    where $\|A\|_2$ denotes the spectral norm of a matrix $A$.
\end{lemma}
\subsection{New New Results}
\begin{definition}[Correlation Decay]
  We say that $\rho$ has $(\gamma,\sigma)$-decay for some
  $\gamma,\sigma\in\RR^{|\Theta|}$ with $\gamma,\sigma>0$ if the following hold.
  \begin{enumerate}
  \item For all $\theta_i\in\Theta$ we have
    $\hat{\rho}_i^{(0,2)}(\theta)<-\gamma_i$ for
    $|\theta-\theta_i|<\sigma_i$.
  \item $\epsilon^{(1,1)}<1$ and
    $\epsilon^{(0,0)}+\epsilon^{(1,0)}\epsilon^{(0,1)}/(1-\epsilon^{(1,1)})
    < 1$.
  \item For $|\theta-\theta_i|<\sigma_i$,
    \begin{equation}
      \frac{(1-\epsilon^{(1,1)})\epsilon_i^{(0,2)}(\theta)+
      \epsilon^{(0,1)}(|\hat{\rho}_i^{(1,2)}(\theta)|+\epsilon_i^{(1,2)}(\theta))}
           {(1-2\epsilon^{(0,0)})(1-\epsilon^{(1,1)})-2\epsilon^{(1,0)}\epsilon^{(0,1)}}
           <\gamma.
    \end{equation}
  \item For $|\theta-\theta_i|\geq\sigma_i$,
    \begin{equation}
      \frac{(1-\epsilon^{(1,1)})(|\hat{\rho}_i(\theta)|+\epsilon_i^{(0,0)}(\theta))
        +\epsilon^{(0,1)}(|\hat{\rho}_i^{(1,0)}(\theta)|+\epsilon_i^{(1,0)}(\theta))}
           {(1-\epsilon^{(0,0)})(1-\epsilon^{(1,1)})-\epsilon^{(1,0)}\epsilon^{(0,1)}}
      <1.
    \end{equation}
  \end{enumerate}
\end{definition}
\begin{definition}[Minimum Separation]
  Suppose $\rho$ has $(\gamma,\sigma)$-decay.
  Define the $i$th normalized
    distance $d_i(\theta)$ for $i=1,\ldots,|\Theta|$ by
  \begin{equation}
    d_i(\theta) := \frac{|\theta_i-\theta|}{\sigma_i}.
  \end{equation}
  We say that $\Theta$ has minimum separation $\Delta$ with respect to
  $\sigma$ if $d_i(\theta_j)\geq \Delta$ for all $i\neq j$.
\end{definition}
\begin{theorem}[Exact Recovery]
  If $\rho$ has $(\gamma,\sigma)$-decay and $\Theta$ has minimum
  separation at least $1$ then Problem \eqref{pr:TVNorm} has $\mu$
  as its unique solution.
\end{theorem}
\subsection{Robustness}


==> relatedworknotes.tex <==

\begin{itemize}
\item I haven't yet emphasized in each bullet how what is stated is
  different from what we do here.
\item In Dossal's PhD thesis he defines
  $$WERC(S) = \frac{\beta(S)}{1-\alpha(S)}$$
  where
  $$\alpha(S) = \sup_{i\in S} \sum_{k\in S,k\neq i}|g_k^Tg_i|$$
  and
  $$\beta(S) = \sup_{j\notin S}\sum_{k\in S}|g_k^Tg_j|.$$
  Here $g_i$ are the columns of the dictionary and $S$ is the support
  of the true signal.  He proves exact recovery occurs when $WERC(S)<1$.
  For arbitrarily finely discretized
  dictionaries, this requires the support atoms to be perfectly
  uncorrelated (i.e., orthogonal).
\item In \cite{murray2017universal} Dragotti and Murray-Bruce use
  frequency estimation techniques to solve phsyics driven SNL
  problems.  Specifically, they approximately express complex
  exponentials as a linear combinations of Green's functions
  translated to each measurement location.  This allows them to cast
  the parameter recovery as a frequency estimation method that can be
  attacked using Prony's method.  The quality of the parameter
  recovery depends on how good their approximation is, and the
  conditioning of the underlying root solving problem.
  Prony's method \cite{deProny:tg} has also been used in
  \cite{vetterli2002sampling,pan2016towards,uriguen2013fri,dragotti2007sampling}
  to solve sparse recovery problems under varying assumptions.
  \bdb{not sure how much I want to say about the other FRI papers
    cited above}
\item The idea of using minimum separation to prove exact recovery
  results was introduced in \cite{superres}, where it is used to study
  the superresolution problem.  To do this they construct a dual
  certificate candidate whose derivatives vanish on the support of the
  true solution.  This style of dual certificate has appeared
  frequently in the literature
  \cite{tang2013atomic,bendory2016robust,peyreduval,bernstein2017deconvolution},
  and motivates our construction here.  In
  \cite{bernstein2017deconvolution} the authors study the
  deconvolution problem for Gaussian and Ricker kernels with irregular
  sampling.  They prove sharp results on when exact recovery is
  possible in terms of the minimum separation, and the proximity of
  the samples to the true support.
\item In
\cite{Tropp:2004vx}, Tropp introduces a new condition for exact
recovery which is support-dependent.  The condition is equivalent to
requiring that the dual certificate candidate with minimum $\ell_2$-norm that
satisfies \eqref{eq:interp1} (but not \eqref{eq:interp2}) is a valid
certificate.  This condition is known to be too weak to prove exact
recovery for super-resolution and deconvolution.
\item In \cite{tang2013atomic} study the deconvolution problem with
  continuous measurements.  Using the dual certificate techniques from \cite{superres}
  they show that by controlling the first 4 derivatives of the
  autocorrelation of the convolution kernel exact recovery is
  achievable via total variation minimization with constant
  separation.  In \cite{bendory2016robust} the same problem is studied
  in 1 and 2 dimensions.  Using a similar dual certificate
  construction, they are able to prove exact recovery with
  constant separation by assuming quadratic decay on the first 3
  derivatives of the convolution kernel.  In \cite{peyreduval} Duval
  and Peyr{\'e} analyze the deconvolution problem in the small noise
  regime, and show that for problems with an appropriate dual
  certificate, total variation minimization can still recover
  the correct number of spikes, and that these estimated spikes
  converge to the true spikes as the noise limits to zero.
\item In \cite{Donoho2197}, Donoho and Elad connect
  the spark of a matrix to sparse recoverability, and then prove
  bounds on the spark using the incoherence of the dictionary.
  In \cite{Tropp:2004gc}, Tropp builds on these results, and extends
  them to show that both orthogonal matching pursuit and basis pursuit
  obtain exact recovery when the number of parameters satisfies
  $(1+1/M(\Phi))/2$ where $M(\Phi)$ is the coherence of the
  dictionary.
\item  In \cite{li2014heat} Li, Osher, and Tsai use sparse recovery
  techniques to identify heat sources from temperature samples.  They
  are able to prove that if a single source is surrounded by
  sufficiently close samples, then it can be recovered robustly (in
  the sense of Wasserstein distance) using $\ell_1$ minimization.
  In \cite{borcea2015resolution}, Borcea and Kocyigit use $\ell_1$
  minimization to locate sources using sound wave receivers.  Using a
  dictionary built from the Green's function of the Helmholtz equation
  they derive a relationship between its coherence, and the resolution
  at which they can resolve the sources.
\item In \cite{Tropp:2006jc} Tropp shows that exact recovery is
  possible when $\|\Phi_{\Theta}^+\Phi_{\Theta^c}\|_1<1$ where
  $\Phi_\Theta$ is the columns of $\Phi$ corresponding to the support
  $\Theta$, $\Phi_{\Theta^c}$ are the remaining columns, and
  $\|\cdot\|_1$ denotes the matrix norm 1-norm (i.e., the largest
  absolute column sum).  This is equivalent to saying the dual
  certificate candidate with minimum
  2-norm that interpolates any sign pattern on the support is a valid
  dual certificate.  While this can be interpretted as a condition
  only relying on support-centered correlations, it is known to be
  strictly weaker than the vanishing-derivative based certificates for
  deconvolution and super-resolution.
\end{itemize}
\subsection{Maybe for Introduction}
\begin{itemize}
\item Maybe in introduction - Applied papers on L1 for EEG, MRF, Ultrasound,Seismology
\item Peyre, Poon, - Correlation Paper (maybe we don't need this)
\item Pieper Paper (hard to read, unclear what to do)
\item Mamonov - Advection
\end{itemize}

